Solving strategies for data-driven one-dimensional elasticity exhibiting nonlinear strains

In this work, we extend and generalize our solving strategy, first introduced in [1], based on a greedy optimization algorithm and the alternating direction method (ADM) for nonlinear systems computed with multiple load steps. In particular, we combine the greedy optimization algorithm with the direct data-driven solver based on ADM which is firstly introduced in [2] and combined with the Newton-Raphson method for nonlinear elasticity in [3]. We numerically illustrate via one- and two-dimensional bar and truss structures exhibiting nonlinear strain measures and different constitutive datasets that our solving strategy generally achieves a better approximation of the globally optimal solution. This, however, comes at the expense of higher computational cost which is scaled by the number of "greedy" searches. Using this solving strategy, we reproduce the first cycle of the cyclic testing for a nylon rope that was performed at industrial testing facilities for mooring lines manufacturers. We also numerically illustrate for a truss structure that our solving strategy generally improves the accuracy and robustness in cases of an unsymmetrical data distribution and noisy data.

==> algorithms/adm.tex <==
\begin{algorithm}
\textbf{Input}:
	data set $\dataset$,
	external force vector $\vect{f}$ \\
\textbf{Output}: $\vect{x}$, $(\hat{\vect{e}}^*, \hat{\vect{s}}^*)$
\begin{algorithmic}[1]
    \State $\vect{x} = \vect{0}$      \Comment{Initial solution guess}
\For{$j$ in $1,\ldots,$number of load steps}
    \State $\vect{f}^{(j)} = \vect{f} * \lambda_j$      \Comment{$j$-th load factor $\lambda_j$}
    \State $i=0$     \Comment{Number of ADM iteration}
    \State \underline{\textit{Step 1}}: Initial data assignment (for the first load step)
    \If{$j=1$}
        \For{$n$ in $1,\ldots,n_e$}
        \State Initialize $(\hat{\vect{e}}^{*(i,j)}, \hat{\vect{s}}^{*(i,j)}) \in \dataset$ randomly, or from the stress-free state, or using nullspace-initialization.
        \EndFor
    \Else
        \State $\hat{\vect{e}}^{*(i,j)} = \hat{\vect{e}}^{*(i,j-1)}$, $\hat{\vect{s}}^{*(i,j)} = \hat{\vect{s}}^{*(i,j-1)}$
    \EndIf    
    \State \underline{\textit{Step 2}}: Newton-Raphson iteration scheme
    \State $k = 0$      \Comment{Number of Newton-Raphson iteration}
    \While{$\Delta\,\vect{x} \,\geq\, 10^{-10}$}        
    	\State Assemble $\mat{A} \left(\vect{x}^{k-1}, \hat{\vect{e}}^{*(j)}, \hat{\vect{s}}^{*(j)} \right)$        
        \State Solve $\mat{A} \left(\vect{x}^{k-1} \right) \, \Delta \vect{x} = \vect{b}\left(\vect{x}^{k-1}, \hat{\vect{e}}^{*(j)}, \hat{\vect{s}}^{*(j)}, \vect{f}^{(j)} \right)$
        \State $\vect{x}^k \,=\, \vect{x}^{k-1} + \Delta\,\vect{x}$
        \State k\,+=\,1
	\EndWhile
    \State $\vect{x}^{(i,j)} = \vect{x}^k$        \Comment{Get the converged solution}
    \State \underline{\textit{Step 3}}: Collect $(\hat{\vect{e}}^{(i,j)},\, \hat{\vect{s}}^{(i,j)})$ from $\vect{x}^{(i,j)}$.
	\State \underline{\textit{Step 4}}: Local state assignment
    \For{$n$ in $1,\ldots,n_e$}
        \State Choose $(\hat{\vect{e}}^{*(i+1,j)}, \hat{\vect{s}}^{*(i+1,j)}) \in \dataset$ s.t. $\frac{c}{2}(\bar{\mathbf{e}}^{(i,j)} - \hat{\vect{e}}^{*(i+1,j)}) + \frac{1}{2c}(\bar{\mathbf{s}}^{(i,j)} - \hat{\vect{s}}^{*(i+1,j)})$ = min.
    \EndFor
    \State \underline{\textit{Step 5}}: Test convergence
    \If{$(\hat{\vect{e}}^{*(i+1,j)}, \hat{\vect{s}}^{*(i+1,j)}) = (\hat{\vect{e}}^{*(i,j)}, \hat{\vect{s}}^{*(i,j)})$ $\forall \, n=1,\ldots,n_e$}
        \State Return $\vect{x}^{(i,j)}$, $(\hat{\vect{e}}^{*(i,j)}, \hat{\vect{s}}^{*(i,j)})$
    \Else
        \State $i \,+=\, 1$
        \State Repeat steps 2-5.
    \EndIf
\EndFor
\caption{Direct data-driven solver based on the Alternating direction method (ADM), combined with the Newton-Raphson iteration scheme.}
\end{algorithmic}
\end{algorithm}

==> sections/section2preliminaries.tex <==



